SoK: Pragmatic Assessment of Machine Learning for Network Intrusion Detection

Machine Learning (ML) has become a valuable asset to solve many real-world tasks. For Network Intrusion Detection (NID), however, scientific advances in ML are still seen with skepticism by practitioners. This disconnection is due to the intrinsically limited scope of research papers, many of which primarily aim to demonstrate new methods ``outperforming'' prior work -- oftentimes overlooking the practical implications for deploying the proposed solutions in real systems. Unfortunately, the value of ML for NID depends on a plethora of factors, such as hardware, that are often neglected in scientific literature. This paper aims to reduce the practitioners' skepticism towards ML for NID by "changing" the evaluation methodology adopted in research. After elucidating which "factors" influence the operational deployment of ML in NID, we propose the notion of "pragmatic assessment", which enable practitioners to gauge the real value of ML methods for NID. Then, we show that the state-of-research hardly allows one to estimate the value of ML for NID. As a constructive step forward, we carry out a pragmatic assessment. We re-assess existing ML methods for NID, focusing on the classification of malicious network traffic, and consider: hundreds of configuration settings; diverse adversarial scenarios; and four hardware platforms. Our large and reproducible evaluations enable estimating the quality of ML for NID. We also validate our claims through a user-study with security practitioners.

==> appendices/tables/template/_baseline.tex <==

\begin{table*}
  \centering
  \caption{\dataset{dataset} baseline results (no temporal dependency).}

    \begin{subtable}[htbp]{1.95\columnwidth}
        \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}{c|c ? cc|cc? cc|cc? cc|cc? cc|cc}
             \multicolumn{2}{c?}{Available Data} & \multicolumn{4}{c?}{Limited (100 per class) [N=1000]} & \multicolumn{4}{c?}{Scarce (20\% of \scbb{D}) [N=100]} &  \multicolumn{4}{c?}{Moderate (40\% of \scbb{D}) [N=100]} &  \multicolumn{4}{c}{Abundant (80\% of \scbb{D}) [N=100]} \\ \hline
             \multicolumn{2}{c?}{Features} &
             \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} & \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} & \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} &  
             \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c}{Essential} \\ \hline
            Alg. & Design & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} \\
             \toprule
             
             \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             
            \midrule
            \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
            
            \bottomrule
        \end{tabular}
        }
                
        \caption{\textit{Baseline} (static): results against `known' attacks seen during the training stage.} 
    \label{tab:_baseline_static}
    \end{subtable}
    
    
    \begin{subtable}[htbp]{1.4\columnwidth}
        \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}{c|c ? cc|cc? cc|cc? cc|cc? cc|cc}
             \multicolumn{2}{c?}{Available Data} & \multicolumn{4}{c?}{Limited (100 per class) [N=1]} & \multicolumn{4}{c?}{Scarce (20\% of \scbb{D}) [N=1]} &  \multicolumn{4}{c?}{Moderate (40\% of \scbb{D}) [N=1]} &  \multicolumn{4}{c}{Abundant (80\% of \scbb{D}) [N=1]} \\ \hline
             \multicolumn{2}{c?}{Features} &
             \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} & \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} & \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} &  
             \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c}{Essential} \\ \hline
            Alg. & Design & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} & \smamath{fpr} & \smamath{tpr} \\
             \toprule
             
             \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             
            \midrule
            \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{6}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB}}} 
             & BD & \\
             & MD & \\
             & ED & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
            
            \bottomrule
        \end{tabular}
        }
                
        \caption{\textit{Baseline} (temporal): results against `known' attacks seen during the training stage.} 
    \label{tab:_baseline_temporal}
    \end{subtable}
    
    
    
    \label{tab:_baseline}
\end{table*}




==> appendices/tables/template/_extra.tex <==
\begin{table*}[!htbp]
  \centering
  \caption{\dataset{CTU13} Multi-classification results.}
        \resizebox{2.0\columnwidth}{!}{
        \begin{tabular}{c|c ? cc|cc? cc|cc? cc|cc? cc|cc}
             \multicolumn{2}{c?}{Labelling} & \multicolumn{4}{c?}{100 (N=1000)} & \multicolumn{4}{c?}{20\% (N=100)} &  \multicolumn{4}{c?}{50\% (N=100)} &  \multicolumn{4}{c}{100\% (N=100)} \\ \hline
             \multicolumn{2}{c?}{Features} &
             \multicolumn{2}{c|}{Extended} & \multicolumn{2}{c?}{Essential} & \multicolumn{2}{c|}{Extended} & \multicolumn{2}{c?}{Essential} & \multicolumn{2}{c|}{Extended} & \multicolumn{2}{c?}{Essential} & \multicolumn{2}{c|}{Extended} & \multicolumn{2}{c}{Essential}  \\ \hline
            Alg. & Arch. & 
            iid & iid? & iid & iid? & 
            iid & iid? & iid & iid? & 
            iid & iid? & iid & iid? & 
            iid & iid? & iid & iid? \\
             \toprule
             
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF}}}
             & MD & \\
             & B+MD & \\ 
             \midrule
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT}}}
             & MD & \\
             & B+MD & \\ 
             \midrule
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR}}}
             & MD & \\
             & B+MD & \\ 
             \midrule
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB}}}
             & MD & \\
             & B+MD & \\ 
             \bottomrule
             \end{tabular} 
             }
             \label{tab:ctu_multi}
\end{table*}


\begin{table*}[!htbp]
  \centering
  \caption{\dataset{CTU13} Training Times.}
        \resizebox{0.7\columnwidth}{!}{
        \begin{tabular}{c|c ? cc? cc? cc? cc}
             \multicolumn{2}{c?}{Labelling} & \multicolumn{2}{c?}{100 (N=1000)} & \multicolumn{2}{c?}{20\% (N=100)} &  \multicolumn{2}{c?}{50\% (N=100)} &  \multicolumn{2}{c}{100\% (N=100)} \\ \hline
              \hline
            Alg. & Arch. & 
            P1 & P2 &
            P1 & P2 &
            P1 & P2 &
            P1 & P2  \\
             \toprule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF (100\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT (2.6\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR (100\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB (100\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             
              
             \bottomrule
             \end{tabular} 
             }
             \label{tab:ctu_training}
\end{table*}

\begin{table*}[!htbp]
  \centering
  \caption{\dataset{CTU13} Inference Time.}
        \resizebox{1.3\columnwidth}{!}{
        \begin{tabular}{c|c ? ccc? ccc? ccc? ccc}
             \multicolumn{2}{c?}{Labelling} & \multicolumn{3}{c?}{100 (N=1000)} & \multicolumn{3}{c?}{20\% (N=100)} &  \multicolumn{3}{c?}{50\% (N=100)} &  \multicolumn{3}{c}{100\% (N=100)} \\ \hline
              \hline
            Alg. & Arch. & 
            P1 & P2 & P3 &
            P1 & P2 & P3 &
            P1 & P2 & P3 &
            P1 & P2 & P3 \\
             \toprule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF (100\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT (2.6\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR (100\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB (100\%)}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
              
             \bottomrule
             \end{tabular} 
             }
             \label{tab:ctu_inference}
\end{table*}

==> appendices/tables/template/_multi.tex <==
\begin{table*}[!htbp]
  \centering
  \caption{\dataset{temp} Multi-classification results.}
        \resizebox{2.0\columnwidth}{!}{
        \begin{tabular}{c|c ? cc|cc? cc|cc? cc|cc? cc|cc}
             \multicolumn{2}{c?}{Available Data} & \multicolumn{4}{c?}{Limited (100 per class)} & \multicolumn{4}{c?}{Scarce (20\% of \scbb{D})} &  \multicolumn{4}{c?}{Moderate (40\% of \scbb{D})} &  \multicolumn{4}{c}{Abundant (80\% of \scbb{D})} \\ \hline
             \multicolumn{2}{c?}{Features} &
             \multicolumn{2}{c|}{Static [N=1000]} & \multicolumn{2}{c?}{Temporal [N=1]} & \multicolumn{2}{c|}{Static [N=1000]} & \multicolumn{2}{c?}{Temporal [N=1]} & \multicolumn{2}{c|}{Static [N=1000]} & \multicolumn{2}{c?}{Temporal [N=1]} & \multicolumn{2}{c|}{Static [N=1000]} & \multicolumn{2}{c?}{Temporal [N=1]}  \\ \hline
            Alg. & Arch. & 
            Complete & Essential & Complete & Essential & 
            Complete & Essential & Complete & Essential & 
            Complete & Essential & Complete & Essential & 
            Complete & Essential & Complete & Essential \\
             \toprule
             
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF}}}
             & MD & \\
             & B+MD & \\ 
             \midrule
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT}}}
             & MD & \\
             & B+MD & \\ 
             \midrule
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR}}}
             & MD & \\
             & B+MD & \\ 
             \midrule
             \multirow{2}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB}}}
             & MD & \\
             & B+MD & \\ 
             \bottomrule
             \end{tabular} 
             }
             \label{tab:_multi}
\end{table*}



==> appendices/tables/template/_open.tex <==


\begin{table*}
  \centering
  \caption{\dataset{tempdata13} Results in open world scenarios (against both adversarial and unknown attacks).}

    \begin{subtable}[htbp]{1.95\columnwidth}
        \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}{c|c ? cc|cc? cc|cc? cc|cc? cc|cc}
\multicolumn{2}{c?}{Available Data} & \multicolumn{4}{c?}{Limited (100 per class) [N=1000]} & \multicolumn{4}{c?}{Scarce (20\% of \scbb{D}) [N=100]} &  \multicolumn{4}{c?}{Moderate (40\% of \scbb{D}) [N=100]} &  \multicolumn{4}{c}{Abundant (80\% of \scbb{D}) [N=100]} \\ \hline
             \multicolumn{2}{c?}{Scenario} &
             \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks} & \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks} & \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks} & \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks}  \\ \hline
            Alg. & Design & 
            \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} & \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} & \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} & \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} \\
             \toprule
             
             \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF}}} 
             & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             
            \midrule
            \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT}}} 
             & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR}}} 
             & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB}}} 
             & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
            
            \bottomrule
        \end{tabular}
        }
                
        \caption{\dataset{tempdata13} Results in the absence of tempporal dependency.} 
    \label{tab:tempdata_open_static}
    \end{subtable}
    
    
    \begin{subtable}[htbp]{1.4\columnwidth}
        \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}{c|c ? cc|cc? cc|cc? cc|cc? cc|cc}
\multicolumn{2}{c?}{Available Data} & \multicolumn{4}{c?}{Limited (100 per class) [N=1]} & \multicolumn{4}{c?}{Scarce (20\% of \scbb{D}) [N=1]} &  \multicolumn{4}{c?}{Moderate (40\% of \scbb{D}) [N=1]} &  \multicolumn{4}{c}{Abundant (80\% of \scbb{D}) [N=1]} \\ \hline
             \multicolumn{2}{c?}{Scenario} &
             \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks} & \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks} & \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks} & \multicolumn{2}{c|}{Adversarial Attacks} & \multicolumn{2}{c?}{Unknown Attacks}  \\ \hline
            Alg. & Design & 
            \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} & \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} & \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} & \footnotesize{$tpr$} \tiny{(org)} & \footnotesize{$tpr$} \tiny{(adv)} & \footnotesize{$fpr$} & \footnotesize{$tpr$} \\
             \toprule
             
             \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{RF}}} 
                          & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             
            \midrule
            \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{DT}}} 
             & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{LR}}} 
             & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
             \midrule
            \multirow{5}{*}{\rotatebox{90}{\parbox{40pt}\centering\textbf{HGB}}} 
             & BD & \\
             & MD & \\
             & ED-f & \\ 
             & ED-v & \\
             & ED-s & \\
             & ED-o & \\
            
            \bottomrule
        \end{tabular}
        }
                
        \caption{\dataset{tempdata13} Results that assume `temporal' dependency between samples.} 
    \label{tab:tempdata_open_temporal}
    \end{subtable}
    
    
    
    \label{tab:tempdata_open}
\end{table*}

==> appendices/tables/template/_testing.tex <==
\begin{table*}[!htbp]
  \centering
  \caption{\dataset{temp}: Runtime (in seconds) for testing (on \scbb{E}) the ML-NIDS on the \textit{high-end} platform..}
        \resizebox{1.2\columnwidth}{!}{
        \begin{tabular}{c|c ? cc? cc? cc? cc}
             \multicolumn{2}{c?}{Available Data} & \multicolumn{2}{c?}{Limited (100 per class)} & \multicolumn{2}{c?}{Scarce (20\% of \scbb{D})} &  \multicolumn{2}{c?}{Moderate (40\% of \scbb{D})} &  \multicolumn{2}{c}{Abundant (80\% of \scbb{D})} \\ 
              \hline
            Alg. & Design & 
            Complete & Essential &
            Complete & Essential &
            Complete & Essential &
            Complete & Essential \\
             \toprule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering \textbf{RF} }}
                & \variable{BD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{MD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED-s} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering \textbf{DT} }}
                & \variable{BD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{MD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED-s} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering \textbf{LR} }}
                & \variable{BD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{MD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED-s} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering \textbf{HGB} }}
                & \variable{BD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{MD} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
                
                & \variable{ED-s} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} & \tabvaluetemp{.} \\
             
              
             \bottomrule
             \end{tabular} 
             }
             \label{tab:_testing}
\end{table*}


==> appendices/tables/template/_training.tex <==

\begin{table*}[!htbp]
  \centering
  \caption{\dataset{temp}: Runtime (in seconds) for training the ML-NIDS on the \textit{high-end} platform..}
        \resizebox{1.5\columnwidth}{!}{
        \begin{tabular}{c|c ? cc? cc? cc? cc}
             \multicolumn{2}{c?}{Available Data} & \multicolumn{2}{c?}{Limited (100 per class) [N=1000]} & \multicolumn{2}{c?}{Scarce (20\% of \smabb{D}) [N=100]} &  \multicolumn{2}{c?}{Moderate (40\% of \smabb{D}) [N=100]} &  \multicolumn{2}{c}{Abundant (80\% of \smabb{D}) [N=100]} \\ 
              \hline
            Alg. {\tiny CPU} & Design & 
            Complete & Essential &
            Complete & Essential &
            Complete & Essential &
            Complete & Essential \\
             \toprule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{RF} \\
                  \tiny{all cores}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{DT} \\
                  \tiny{one core}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{LR} \\
                  \tiny{all cores}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{HGB} \\
                  \tiny{all cores}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             
              
             \bottomrule
             \end{tabular} 
             }
             \label{tab:_training}
\end{table*}


==> appendices/tables/template/hardware.tex <==


\begin{table*}
  \centering
  \caption{Runtime (training and testing) on the other platforms (for the \dataset{GTCS} dataset).}

    \begin{subtable}[htbp]{1.95\columnwidth}
        \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}{c|c ? cc|cc? cc|cc? cc|cc? cc|cc}
             \multicolumn{2}{c?}{Available Data} & \multicolumn{4}{c?}{Limited (100 per class)} & \multicolumn{4}{c?}{Scarce (20\% of \smabb{D})} &  \multicolumn{4}{c?}{Moderate (40\% of \smabb{D})} &  \multicolumn{4}{c}{Abundant (80\% of \smabb{D})} \\ 
              \hline
              
            \multicolumn{2}{c?}{Feature Set} & 
            \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} &
            \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} &
            \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c?}{Essential} &
            \multicolumn{2}{c|}{Complete} & \multicolumn{2}{c}{Essential} \\ \hline
              
            Alg. {\tiny CPU} & Design & 
            Train & Test &
            Train & Test &
            Train & Test &
            Train & Test &
            Train & Test &
            Train & Test &
            Train & Test &
            Train & Test \\
             \toprule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{RF} \\
                  \tiny{all cores}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{DT} \\
                  \tiny{one core}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{LR} \\
                  \tiny{all cores}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             \midrule
             
             \multirow{4}{*}{\rotatebox{90}{\parbox{40pt}\centering
             \begin{tabular}{c}
                  \textbf{HGB} \\
                  \tiny{all cores}
             \end{tabular}}}
             & BD & \\
             & MD & \\ 
             & ED & \\ 
             & ED-s & \\ 
             
              
             \bottomrule
             \end{tabular} 
             }
                     \caption{Laptop} 
             \label{tab:_hardware}
             
            \end{subtable}
            

            
\end{table*}

